Is ChatGPT a Good Sentiment Analyzer? A Preliminary Study

Recently, ChatGPT has drawn great attention from both the research community and the public. We are particularly interested in whether it can serve as a universal sentiment analyzer. To this end, in this work, we provide a preliminary evaluation of ChatGPT on the understanding of \emph{opinions}, \emph{sentiments}, and \emph{emotions} contained in the text. Specifically, we evaluate it in three settings, including \emph{standard} evaluation, \emph{polarity shift} evaluation and \emph{open-domain} evaluation. We conduct an evaluation on 7 representative sentiment analysis tasks covering 17 benchmark datasets and compare ChatGPT with fine-tuned BERT and corresponding state-of-the-art (SOTA) models on them. We also attempt several popular prompting techniques to elicit the ability further. Moreover, we conduct human evaluation and present some qualitative case studies to gain a deep comprehension of its sentiment analysis capabilities.

==> table/COQE-Camera.tex <==
\begin{table}
	\centering
	\resizebox{.5\textwidth}{!}{
	\begin{tabular}{c|cccc}
		\hline & \textbf{Car-COQE} & \textbf{Ele-COQE} & \textbf{Camera-COQE}\\ \hline
		\#Subject & 1520 & 950  & 1649 \\	
	    \#Object & 2121 & 1980 & 1316 \\
		\#Aspect & 1917 & 1602 & 1368 \\
		\#Opinion & 2171 & 2089 & 2163 \\
		\#Preference & 2695 & 2289 & 2442 \\
		\hline
		\#Comparative & 1747 & 1800 & 1705 \\	
	    \#Non-Comparative & 1800 & 1800 & 1599 \\
		\#Multi-Comparisons & 550 & 361 & 500 \\ \hline
		\#Comparisons Per Sent & 1.5 & 1.3 & 1.4 \\
		\hline
	\end{tabular}
	}
	\caption{\label{elements}Statistics of three COQE datasets.}
\end{table}

==> table/ECE-ECPE-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\renewcommand{\arraystretch}{1.1}
\centering
\scalebox{0.9}{
\begin{tabular}{llccc}
\toprule
\textbf{Task}         & \textbf{Models}    & \textbf{P}     & \textbf{R}     & \textbf{F1}    \\ \midrule
\multirow{4}{*}{ECE}  & \multicolumn{4}{l}{\cellcolor[HTML]{D9D9D9}\emph{Fine-tuned Results}}                                        \\
                      & PAE-DGL\,$^\dag$            & 75.25          & 64.50           & 69.46          \\
                      
                      & \multicolumn{4}{l}{\cellcolor[HTML]{D9D9D9}\emph{Zero-shot  Results}}                                         \\
                      & ChatGPT            & 75.68          & 72.41          & 74.01          \\ \midrule
\multirow{4}{*}{ECPE} & \multicolumn{4}{l}{\cellcolor[HTML]{D9D9D9}\emph{Fine-tuned  Results}}                                        \\
                      & ECPE-2D\,$^\dag$            & 69.89          & 56.03          & 62.20          \\
                      & \multicolumn{4}{l}{\cellcolor[HTML]{D9D9D9}\emph{Zero-shot  Results}}                                         \\
                      & ChatGPT            & 54.13          & 50.86          & 52.44          \\ \bottomrule
\end{tabular}}
\caption{Comparison results between ChatGPT and baseline models on ECE and ECPE measured by micro F1 score. $\dag$ denotes the results are obtained by re-running experiments based on our evaluation setup.}
\label{tab:ece-ecpe-results}
\end{table}



==> table/open_domain_absc_results.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.1}
\scalebox{0.80}{
\begin{tabular}{lcccccccccc}
\toprule
 &
  \multicolumn{8}{c}{\textbf{Fine-tuned BERT}} &
  \multicolumn{2}{c}{\textbf{ChatGPT}} \\ \cmidrule(r){2-9} \cmidrule(r){10-11}
 & 
  \multicolumn{2}{c}{\textbf{14-Res.}} &
  \multicolumn{2}{c}{\textbf{14-Lap.}} &
  \multicolumn{2}{c}{\textbf{The Rest}} &
  \multicolumn{2}{c}{{\color[HTML]{808080}\textbf{Domain-Specific}}} &
  \multicolumn{2}{c}{\textbf{Zero-shot}} \\ \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11}
\multirow{-3}{*}[1.2ex]{ \makecell*[l]{\textbf{Trained on $\to$} \\ \textbf{Evaluated on $\downarrow$} } }
&
  \textbf{Acc.} &
  \textbf{F1} &
  \textbf{Acc.} &
  \textbf{F1} &
  \textbf{Acc.} &
  \textbf{F1} &
  {\color[HTML]{808080}\textbf{Acc.}} &
  {\color[HTML]{808080}\textbf{F1}} &
  \textbf{Acc.} &
  \textbf{F1} \\ \midrule
14-Res. &
  {\color[HTML]{808080} 81.11} &
  {\color[HTML]{808080} 74.99} &
  \textbf{84.44} &
  \textbf{78.76} &
  80.00 &
  69.63 &
  {\color[HTML]{808080} 81.11} &
  {\color[HTML]{808080} 74.99} &
  {\color[HTML]{00B050} 83.33} &
  61.16 \\
14-Lap. &
  \textbf{77.78} &
  \textbf{70.60} &
  {\color[HTML]{808080} 77.78} &
  {\color[HTML]{808080} 72.84} &
  76.67 &
  59.83 &
  {\color[HTML]{808080} 77.78} &
  {\color[HTML]{808080} 72.84} &
  73.33 &
  53.41 \\
Books &
  57.78 &
  41.91 &
  57.78 &
  42.84 &
  \textbf{62.22} &
  46.11 &
  {\color[HTML]{808080} 71.11} &
  {\color[HTML]{808080} 57.17} &
  {\color[HTML]{00B050} 60.00} &
  {\color[HTML]{00B050} \textbf{51.25}} \\
Clothing &
  74.44 &
  55.00 &
  \textbf{76.67} &
  56.21 &
  \textbf{76.67} &
  \textbf{61.66} &
  {\color[HTML]{808080} 80.00} &
  {\color[HTML]{808080} 58.15} &
  70.00 &
  {\color[HTML]{00B050} 59.65} \\
Hotel &
  86.67 &
  77.59 &
  86.67 &
  76.94 &
  85.56 &
  75.34 &
  {\color[HTML]{808080} 87.78} &
  {\color[HTML]{808080} 77.98} &
  {\color[HTML]{00B050} \textbf{86.67}} &
  {\color[HTML]{00B050} \textbf{83.18}} \\
Device &
  86.67 &
  85.35 &
  86.67 &
  88.92 &
  94.44 &
  98.11 &
  {\color[HTML]{808080} 100.00} &
  {\color[HTML]{808080} 100.00} &
  {\color[HTML]{00B050} \textbf{96.67}} &
  {\color[HTML]{00B050} \textbf{98.89}} \\
Service &
  71.11 &
  67.91 &
  71.11 &
  67.59 &
  \textbf{81.11} &
  \textbf{79.29} &
  {\color[HTML]{808080} 74.44} &
  {\color[HTML]{808080} 62.69} &
  {\color[HTML]{00B050} 76.67} &
  65.30 \\
14-Twitter &
  62.22 &
  54.11 &
  62.22 &
  56.16 &
  \textbf{70.00} &
  \textbf{67.83} &
  {\color[HTML]{808080} 62.22} &
  {\color[HTML]{808080} 60.99} &
  {\color[HTML]{00B050} 66.67} &
  {\color[HTML]{00B050} 64.22} \\
Finance &
  75.56 &
  62.75 &
  74.44 &
  55.59 &
  31.11 &
  31.58 &
  {\color[HTML]{808080} 82.22} &
  {\color[HTML]{808080} 79.07} &
  {\color[HTML]{00B050} \textbf{86.67}} &
  {\color[HTML]{00B050} \textbf{72.35}} \\
METS-Cov &
  53.33 &
  47.06 &
  50.00 &
  37.56 &
  38.89 &
  35.65 &
  {\color[HTML]{808080} 61.11} &
  {\color[HTML]{808080} 58.53} &
  {\color[HTML]{00B050} \textbf{76.67}} &
  {\color[HTML]{00B050} \textbf{55.56}} \\ \midrule
Average &
  72.67 &
  61.14 &
  72.78 &
  60.78 &
  69.67 &
  59.99 &
  {\color[HTML]{808080} 77.78} &
  {\color[HTML]{808080} 67.64} &
  {\color[HTML]{00B050} \textbf{77.67}} &
  {\color[HTML]{00B050} \textbf{66.50}} \\ \bottomrule
\end{tabular}}
\caption{Performance comparison between ChatGPT and fine-tuned BERT for ABSC task on open-domain evaluation.  We also report the domain (dataset)-specific fully-supervised results (in  \textcolor{gray}{gray}) of BERT for reference (denoted by \textcolor{gray}{Domain-Specific}). \texttt{The Rest} denotes that the model is trained on training datasets from 9 domains other than the evaluation test set. The best results (except for fully-supervised results) are in \textbf{bold}. The results in \textcolor{color8}{green} indicate that ChatGPT is at least better than one of the fine-tuned BERT models (based on 14-Restaurant (\texttt{14-Res.}), 14-Laptop (\texttt{14-Lap.}), and 9 datasets (\texttt{The Rest}), respectively).}
\label{tab:open-domain-absc-results}
\end{table*}

==> table/open_domain_aspe_results.tex <==


\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\scalebox{0.9}{
\begin{tabular}{l m{1.5cm}<{\centering} m{1.5cm}<{\centering} m{1.5cm}<{\centering}  m{1.5cm}<{\centering} m{1.5cm}<{\centering} m{1.5cm}<{\centering}}
\toprule

% 
\multirow{2}{*}[-1.5ex]{\makecell*[l]{\textbf{Trained on $\to$} \\ \textbf{Evaluated on $\downarrow$}  } }  &

  \multicolumn{4}{c}{\textbf{Fine-tuned BERT}} &
\multicolumn{2}{c}{\textbf{Zero-shot ChatGPT}} \\ \cmidrule(r){2-5} \cmidrule(r){6-7}
 &
  \textbf{14-Rest.} &
  \textbf{14-Lap.} &
  \textbf{The Rest} &  %\makecell{Domain \\ Specific}
  \textcolor{gray}{\textbf{Domain-Specific}} &
  \textbf{\makecell{Auto \\ Eval.}} & \textcolor{blue2}{\textbf{\makecell{Human \\ Eval.}}} \\ \midrule
14-Restaurant     & \textcolor{gray}{76.55} & 55.06 & 71.10 & \textcolor{gray}{76.55} & \textbf{\textcolor{color8}{72.73}} & \textcolor{blue2}{82.22}\\

14-Laptop     & 43.57 & \textcolor{gray}{68.02} & \textbf{59.36} & \textcolor{gray}{68.02} & \textcolor{color8}{45.45} & \textcolor{blue2}{64.00}    \\

Books      & 38.35 & 25.93 & \textbf{46.64} & \textcolor{gray}{61.17} & 21.92 & \textcolor{blue2}{29.41}  \\

Clothing   & 29.57 & 26.28 & \textbf{50.72} & \textcolor{gray}{67.97} & 25.71 & \textcolor{blue2}{34.78}       \\

Hotel      & 64.07 & 53.21 & \textbf{74.85} & \textcolor{gray}{88.67} & 50.60 & \textcolor{blue2}{62.50}       \\

Device     & 50.74 & \textbf{60.19} & 58.87 & \textcolor{gray}{75.39} & 41.86 & \textcolor{blue2}{69.23}       \\

Service    & 27.01 & 27.03 & \textbf{47.67} & \textcolor{gray}{57.83} & \textcolor{color8}{45.78} & \textcolor{blue2}{63.89}  \\

14-Twitter & \makebox[5ex][r]{1.67}  & \makebox[5ex][r]{3.43}  & \textbf{42.90} & \textcolor{gray}{78.84} & \textcolor{color8}{19.18} &  \textcolor{blue2}{52.63}   \\

Finance    & \makebox[5ex][r]{7.74}  & \makebox[5ex][r]{7.11}  & 14.21 & \textcolor{gray}{79.32} & \textbf{\textcolor{color8}{38.36}} & \textcolor{blue2}{76.92}  \\

METS-Cov   & \makebox[5ex][r]{3.27}  & \makebox[5ex][r]{5.14}  & \textbf{10.27} & \textcolor{gray}{71.71} & \makebox[4.5ex][r]{\textcolor{color8}{3.92}} & \makebox[4.9ex][r]{\textcolor{blue2}{9.88}}  \\ \midrule

Average        & 34.25 & 33.14 & \textbf{47.66} & \textcolor{gray}{72.55} & \textcolor{color8}{36.55} & \textcolor{blue2}{54.55}  \\ \bottomrule
\end{tabular}}
\label{tab:open-domain-aspe-results}
\caption{Performance comparison between ChatGPT and BERT for E2E-ABSA task on the open-domain evaluation. We report the domain/dataset-specific fully-supervised results (in \textcolor{gray}{gray}) of BERT for reference (denoted by \textcolor{gray}{Domain-Specific}). \texttt{The Rest} denotes that the model is trained on training datasets from 9 domains other than the evaluation test set. The results in \textcolor{color8}{green} indicate that ChatGPT is at least better than one of the fine-tuned BERT models (based on 14-Restaurant (\texttt{14-Res.}), 14-Laptop (\texttt{14-Lap.}), and 9 datasets (\texttt{The Rest}), respectively). We also report the human evaluation results of ChatGPT for reference (in \textcolor{blue2}{blue}). The best results (except for fully-supervised results and human evaluation results) are in \textbf{bold}.}
\end{table*}







==> table/standard-eval-dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.1}
\scalebox{0.9}{
\begin{tabular}{llc}
\toprule
\textbf{Task}         & \textbf{Dataset} & \textbf{\#Test} \\ \midrule
SC                    & SST-2            & \makebox[4ex][r]{872}             \\ \midrule
\multirow{2}{*}{ABSC} & 14-Restaurant           & \makebox[4ex][r]{1119}            \\
                      & 14-Laptop          & \makebox[4ex][r]{632}             \\ \midrule
\multirow{2}{*}{E2E-ABSA} & 14-Restaurant          & \makebox[4ex][r]{496}             \\
                      & 14-Laptop           & \makebox[4ex][r]{339}             \\ \midrule

CSI                    & Camera            & \makebox[4ex][r]{661}\\
CEE                    & Camera            & \makebox[4ex][r]{341}\\ \midrule
ECE  & Emotion-Cause-Dataset & 100 \\
ECPE  & Emotion-Cause-Dataset & 100 \\ 
                    \bottomrule

\end{tabular}}
\caption{The tasks and datasets involved in the standard evaluation. \#Test denotes the number of examples used for evaluation.}
\label{tab:standard-eval-datasets}
\end{table}


==> table/standard_aspe_human_eval.tex <==
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{14-Rest.} & \textbf{14-Laptop} \\ \midrule
\multicolumn{3}{l}{\cellcolor[HTML]{D9D9D9}\emph{Fully-supervised results}}       \\
BERT           & 77.75           & 66.05           \\
SOTA\,$ ^\delta$           & 78.68            & 70.32          \\ \midrule
\multicolumn{3}{l}{\cellcolor[HTML]{D9D9D9}\emph{Zero-shot results}}              \\
ChatGPT  (Auto Eval.)        & 69.14           & 49.11           \\

ChatGPT (Human Eval.)       & \textcolor{blue2}{83.86} 	 & \textcolor{blue2}{72.77}           \\ 

\bottomrule
\end{tabular}}
\caption{The human evaluation results (in \textcolor{blue2}{blue}) of ChatGPT on the E2E-ABSA task. $\delta$ denotes the model performance reported in~\citet{DBLP:conf/ijcai/0001LLWLJ22-SyMux} on this task. }
\label{tab:standard_aspe_human_eval}
\end{table}
